Certifiably Robust Policies for Uncertain Parametric Environments

We present a data-driven approach for producing policies that are provably robust across unknown stochastic environments. Existing approaches can learn models of a single environment as an interval Markov decision processes (IMDP) and produce a robust policy with a probably approximately correct (PAC) guarantee on its performance. However these are unable to reason about the impact of environmental parameters underlying the uncertainty. We propose a framework based on parametric Markov decision processes (MDPs) with unknown distributions over parameters. We learn and analyse IMDPs for a set of unknown sample environments induced by parameters. The key challenge is then to produce meaningful performance guarantees that combine the two layers of uncertainty: (1) multiple environments induced by parameters with an unknown distribution; (2) unknown induced environments which are approximated by IMDPs. We present a novel approach based on scenario optimisation that yields a single PAC guarantee quantifying the risk level for which a specified performance level can be assured in unseen environments, plus a means to trade-off risk and performance. We implement and evaluate our framework using multiple robust policy generation methods on a range of benchmarks. We show that our approach produces tight bounds on a policy's performance with high confidence.

==> Figures/inducedValueFig.tex <==
% Define beta distribution function
\usetikzlibrary{math}



% \begin{tikzpicture}[baseline]
% \begin{axis}[width=2.2in,
%              height=1.9in,
%              ymin=0,
%              ymax=2,
%              xmin=-0.01,
%              xmax=1.01,
%              xlabel={$\theta$},
%              ylabel={$\Pr$},
%              xtick={0, 0.25, 0.5, 0.75, 1},
%              ylabel style={rotate=-90, xshift=10pt}, % Rotate and move closer to the axis
%              smooth,
%              samples=200,
%              clip=true]
% \addplot[mark=none, unbounded coords=jump, color=	alizarin, line width = 1.2pt, fill = antiquewhite] coordinates {
%                 (0,0)
%                 (0.1,0)
%                 (0.2,0.5)
%                 (0.28,0.8)
%                 (0.42,0.7)
%                 (0.6,1.48)
%                 (0.7,1.5)
%                 (0.8,1.1)
%                 (0.9,0.5)
%                 (1.0,0)
%             };
% \end{axis}
% \node[] at (1,1.5) {$\mathbb{P}$};
% \end{tikzpicture}

\scalebox{0.45}{
\begin{minipage}{0.6\textwidth}
\begin{tikzpicture}[baseline, remember picture]
\begin{axis}[width=2.2in,
             height=1.9in,
             ymin=0,
             ymax=2,
             xmin=-0.01,
             xmax=1.01,
             xlabel={$\theta$},
             ylabel={$\Pr$},
             xtick={0, 0.25, 0.5, 0.75, 1},
             ylabel style={rotate=-90, xshift=10pt}, % Rotate and move closer to the axis
             smooth,
             samples=200,
             clip=true]
\addplot[mark=none, unbounded coords=jump, color=alizarin, line width = 1.2pt, fill = antiquewhite] coordinates {
                (0,0)
                (0.1,0)
                (0.2,0.6)
                (0.28,0.9)
                (0.42,0.8)
                (0.6,1.58)
                (0.7,1.6)
                (0.8,1.2)
                (0.9,0.6)
                (1.0,0)
            };
\end{axis}
\node[] at (1,1.7) {$\mathbb{P}$};
\node[] (left) at (4,1.65) {};
\end{tikzpicture}
\end{minipage}
\begin{minipage}{0.4\textwidth}
\begin{tikzpicture}[baseline, remember picture]
\begin{axis}[width=2.2in,
             height=1.9in,
             ymin=0,
             ymax=4,
             xmin=-0.01,
             xmax=3.01,
             xlabel={$V(\pi_1, \theta)$},
             ylabel={$\Pr$},
             xtick={0, 0.5, 1, 1.5, 2, 2.5, 3},
             ylabel style={rotate=-90, xshift=10pt}, % Rotate and move closer to the axis
             smooth,
             samples=200,
             clip=true]
\addplot[mark=none, unbounded coords=jump, color=alizarin, line width = 1.2pt, fill = offwhite] coordinates {
                (0,-1)
                (0.3,-1)
                (0.6,-1)
                (0.84,-1)
                (1.26,0.4)
                (1.7,2)
                (2.0, 1.3)
                (2.35,3.3)
                (2.7,0.8)
                (3.0,0)
            };
\draw[dashed, darkgray] (axis cs:1.14,0) -- (axis cs:1.14,4.01);
\end{axis}
\node[] at (1.5,3.6) {$V(\pi_1)$};
\node[] (upper) at (-1,0.5) {};
\end{tikzpicture}
\vspace{0.5cm}

\begin{tikzpicture}[baseline, remember picture]
\definecolor{color1}{rgb}{0.1,0.498039215686275,0.9549019607843137}

\begin{axis}[width=2.2in,
             height=1.9in,
             ymin=0,
             ymax=2,
             xmin=-0.01,
             xmax=3.01,
             xlabel={$V(\pi_2, \theta)$},
             ylabel={$\Pr$},
             xtick={0, 0.5, 1, 1.5, 2, 2.5, 3},
             ylabel style={rotate=-90, xshift=10pt}, % Rotate and move closer to the axis
             smooth,
             samples=200,
             clip=true]
\addplot[mark=none, unbounded coords=jump, color=alizarin, line width = 1.2pt, fill = offwhite] coordinates {
                (0,0.0)
                (0.3,0.01)
                (0.8,1.68)
                (1.4,0.8)
                (1.8,1.2)
                (2.4, 0.25)
                (3.0,0.01)
            };
\draw[dashed, darkgray] (axis cs:0.29,0) -- (axis cs:0.29,2.01);

\end{axis}
\node[] at (0.5,3.6) {$V(\pi_2)$};
\node[] (lower) at (-1,2.625) {};
\end{tikzpicture}
\end{minipage}

% Draw arrows with labels
\begin{tikzpicture}[overlay, remember picture]
  \draw[->, darkgray, line width=1pt] ([shift=({0.2,0.3})]left.east) -- (upper.west) node[midway, above, sloped] {$\pi_1$};
  \draw[->, darkgray, line width=1pt] ([shift=({0.2,-0.3})]left.east) -- (lower.west) node[midway, below, sloped] {$\pi_2$};
\end{tikzpicture}
}



==> Figures/upmdp_figure.tex <==
\begin{tikzpicture}[node distance = 3cm, on grid, auto]
    \scalebox{0.72}{
        \node (q0) [state,initial by arrow, initial where = above left ,initial text = {}] {$s_0$};
        \node (q1) [state,initial text = {},right = of q0] {$s_1$};
        \node (q2) [state, below  = of q0, label =above:$ $] {$s_2$};
        \node (q3) [state, below  = of q1, label =below:$ $] {$s_3$};
        % \node (q4) [state, below right = of q1, label =below:$ $] {$s_4$};

        \node (s1) [draw,circle, fill = antiquewhite, right = 0.0 and 1.2 of q0, inner sep = 2pt] {};
        \node (s2) [draw,circle, fill = antiquewhite, below = 1.2 and 0.0 of q0, inner sep = 2pt] {};

        \path[thick] 
            (q0) edge node[below] {$\alpha$}   (s1)
            (q0) edge node {$\alpha$}  (s2);
        \path [-stealth, thick]
        
            (s1) edge [bend left = 0] node [yshift = 0pt, xshift = 0pt] {\footnotesize$q^3+ 0.2$}   (q1)
            (s1) edge [right,bend left = 10] node [xshift=1pt, yshift = 2pt] {\small$p$}   (q3)
             (s1.north) edge [right ,bend right =60] node [xshift=-30pt, yshift = 10pt] {\footnotesize$0.8-p-q^3$}   (q0)

            (s2) edge [right, bend left = 0] node [yshift = 0pt, xshift = 0pt, left] {\footnotesize$r$}   (q2)
            (s2) edge [bend right = 10] node [left] [xshift=-3pt, yshift = -4pt] {\small$p$}   (q3)
             (s2.west) edge [left ,bend left =60] node [xshift=-1pt, yshift = 2pt] {\footnotesize$1-p-r$}   (q0)

            % (s2) edge [bend left = 0] node [yshift = 0pt, xshift = 0pt] {\small$r$}   (q3)
            % (s2) edge [right,bend left = 10] node [xshift=1pt, yshift = 2pt] {\small$p$}   (q4)
            % (s2) edge [right,bend right =10] node [xshift=-6pt, yshift = -9pt] {\footnotesize$1-p-r$}   (q2)

        
            (q2) edge [loop right]  node {$\beta$}()
            (q3) edge [loop right]  node {$\alpha$}()
            (q1) edge [loop right]  node {$\beta$}(); 
            }
    \end{tikzpicture}
